Gaussians Can Subtract: Neural Dissolve Fields for Hybrid Scene Rendering

Hybrid Mesh-Gaussian rendering combines compact textured surfaces with flexible 3D Gaussian primitives, offering an efficient alternative to purely Gaussian scene representations for structured environments. Existing scene-reconstruction hybrids commonly follow an additive formulation, where Gaussian residuals compensate for errors left by the mesh. However, not every Mesh-Gaussian conflict is caused by missing content: residual geometry errors, occlusion mismatch, texture-projection artifacts, and view-dependent appearance can make the same mesh content consistent in one view but inconsistent in another. We therefore formulate hybrid rendering as a multi-view inconsistency problem and present Gaussolve, a subtract-and-refill framework that selectively dissolves inconsistent mesh content before residual Gaussians refill the revealed regions. We introduce a lightweight Neural Dissolve Field, parameterized by scalar spherical-harmonic Gaussians, to learn where and from which viewing directions mesh content should be dissolved. A continuous transmittance fusion rule progressively exposes residual Gaussians behind the dissolved mesh, preserving their reconstruction gradients and avoiding hard visibility discontinuities. Experiments on structured and semi-structured scenes demonstrate higher visual fidelity with fewer Gaussian primitives and faster rendering. Project page: https://ooosn.github.io/gaussians-can-subtract/

==> exp1.tex <==
\def\gtW{0.216\textwidth}    
\def\methW{0.126\textwidth} 

\newcommand{\setboxes}[8]{%
  \xdef\RxA{#1}\xdef\RyA{#2}\xdef\RxB{#3}\xdef\RyB{#4}%
  \xdef\BxA{#5}\xdef\ByA{#6}\xdef\BxB{#7}\xdef\ByB{#8}%
}

\newcommand{\datasetlabel}[1]{%
  \llap{%
    \rotatebox[origin=c]{90}{\textbf{#1}}%
    \hspace{1em}%
  }%
}

\newcommand{\gtbox}[1]{%
  \begin{minipage}[c]{\gtW}
    \resizebox{\linewidth}{!}{%
      \begin{tikzpicture}[x=1bp,y=1bp]
        \node[anchor=south west,inner sep=0] at (0,0) {\includegraphics{#1}};
        \draw[red, ultra thick] (\RxA,\RyA) rectangle (\RxB,\RyB);
        \draw[blue, ultra thick] (\BxA,\ByA) rectangle (\BxB,\ByB);
      \end{tikzpicture}%
    }
  \end{minipage}%
}

\newcommand{\patchcol}[1]{%
  \begin{minipage}[c]{\methW}
    \includegraphics[viewport={\RxA} {\RyA} {\RxB} {\RyB}, clip, width=\linewidth]{#1}\\[0.5pt]
    \includegraphics[viewport={\BxA} {\ByA} {\BxB} {\ByB}, clip, width=\linewidth]{#1}
  \end{minipage}%
}

\newcommand{\patchcoll}[1]{%
  \begin{minipage}[c]{\methW}
    \includegraphics[viewport={\RxA} {\RyA} {\RxB} {\RyB}, clip, width=\linewidth]{images/main_experiment/gaussolve-r/5.png}\\[0.5pt]
    \includegraphics[viewport={\BxA} {\ByA} {\BxB} {\ByB}, clip, width=\linewidth]{#1}
  \end{minipage}%
}

\newcommand{\patchcolll}[1]{%
  \begin{minipage}[c]{\methW}
    \includegraphics[viewport={\RxA} {\RyA} {\RxB} {\RyB}, clip, width=\linewidth]{images/main_experiment/hardz/111.jpg}\\[0.5pt]
    \includegraphics[viewport={\BxA} {\ByA} {\BxB} {\ByB}, clip, width=\linewidth]{#1}
  \end{minipage}%
}

\begin{figure*}[!t]
\centering
\small
\setlength{\tabcolsep}{1pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c@{\hspace{0.4em}}ccccccc@{}}
& \textbf{Reference} & \textbf{GT} & \textbf{3DGS} & \textbf{PGSR} & \textbf{3D-GES} & \textbf{MeshSplatting} & \textbf{Ours} \\
\addlinespace[0.5pt]

\setboxes{340}{300}{490}{390}{600}{160}{750}{250}
\rotatebox[origin=c]{90}{\textbf{ML-Hypersim-001}} &
\gtbox{images/main_experiment/gt/1.jpg} &
\patchcol{images/main_experiment/gt/1.jpg} &
\patchcol{images/main_experiment/3dgs/1.jpg} &
\patchcol{images/main_experiment/PGSR/1.jpg} &
\patchcol{images/main_experiment/ges/1.jpg} &
\patchcol{images/main_experiment/MeshSplatting/1.jpg} &
\patchcol{images/main_experiment/gaussolve-s/1.jpg} \\
\addlinespace[4pt]

\setboxes{000}{518}{120}{590}{280}{440}{430}{530}
\rotatebox[origin=c]{90}{\textbf{Playroom}} &
\gtbox{images/main_experiment/gt/2.jpg} &
\patchcol{images/main_experiment/gt/2.jpg} &
\patchcol{images/main_experiment/3dgs/2.jpg} &
\patchcol{images/main_experiment/PGSR/2.jpg} &
\patchcol{images/main_experiment/ges/2.jpg} &
\patchcol{images/main_experiment/MeshSplatting/2.jpg} &
\patchcol{images/main_experiment/hardz/2.jpg} \\
\addlinespace[4pt]

\setboxes{100}{50}{250}{140}{640}{610}{790}{700}
\rotatebox[origin=c]{90}{\textbf{SaintAnne}} &
\gtbox{images/main_experiment/gt/3.jpg} &
\patchcol{images/main_experiment/gt/3.jpg} &
\patchcol{images/main_experiment/3dgs/3.jpg} &
\patchcol{images/main_experiment/PGSR/3.jpg} &
\patchcol{images/main_experiment/ges/3.jpg} &
\patchcol{images/main_experiment/MeshSplatting/3.jpg} &
\patchcol{images/main_experiment/gaussolve-s/3.jpg} \\
\addlinespace[4pt]



\end{tabular}%
}
\caption{\textbf{Qualitative comparisons on novel-view synthesis.} Compared with 3DGS, PGSR, 3D-GES, and MeshSplatting, Gaussolve better preserves weakly textured surfaces. The red and blue boxes indicate the corresponding enlarged regions.}
\label{main_exp}
\end{figure*}

==> exp12.tex <==
\def\gtW{0.216\textwidth}    
\def\methW{0.126\textwidth} 

\providecommand{\setboxes}[8]{%
  \xdef\RxA{#1}\xdef\RyA{#2}\xdef\RxB{#3}\xdef\RyB{#4}%
  \xdef\BxA{#5}\xdef\ByA{#6}\xdef\BxB{#7}\xdef\ByB{#8}%
}

\providecommand{\datasetlabel}[1]{%
  \llap{%
    \rotatebox[origin=c]{90}{\textbf{#1}}%
    \hspace{1em}%
  }%
}

\providecommand{\gtbox}[1]{%
  \begin{minipage}[c]{\gtW}
    \resizebox{\linewidth}{!}{%
      \begin{tikzpicture}[x=1bp,y=1bp]
        \node[anchor=south west,inner sep=0] at (0,0) {\includegraphics{#1}};
        \draw[red, ultra thick] (\RxA,\RyA) rectangle (\RxB,\RyB);
        \draw[blue, ultra thick] (\BxA,\ByA) rectangle (\BxB,\ByB);
      \end{tikzpicture}%
    }
  \end{minipage}%
}

\providecommand{\patchcol}[1]{%
  \begin{minipage}[c]{\methW}
    \includegraphics[viewport={\RxA} {\RyA} {\RxB} {\RyB}, clip, width=\linewidth]{#1}\\[0.5pt]
    \includegraphics[viewport={\BxA} {\ByA} {\BxB} {\ByB}, clip, width=\linewidth]{#1}
  \end{minipage}%
}

\providecommand{\patchcoll}[1]{%
  \begin{minipage}[c]{\methW}
    \includegraphics[viewport={\RxA} {\RyA} {\RxB} {\RyB}, clip, width=\linewidth]{images/main_experiment/gaussolve-r/5.png}\\[0.5pt]
    \includegraphics[viewport={\BxA} {\ByA} {\BxB} {\ByB}, clip, width=\linewidth]{#1}
  \end{minipage}%
}

\providecommand{\patchcolll}[1]{%
  \begin{minipage}[c]{\methW}
    \includegraphics[viewport={\RxA} {\RyA} {\RxB} {\RyB}, clip, width=\linewidth]{images/main_experiment/hardz/111.jpg}\\[0.5pt]
    \includegraphics[viewport={\BxA} {\ByA} {\BxB} {\ByB}, clip, width=\linewidth]{#1}
  \end{minipage}%
}

\begin{figure*}[!t]
\centering
\small
\setlength{\tabcolsep}{1pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c@{\hspace{0.4em}}ccccccc@{}}
& \textbf{Reference} & \textbf{GT} & \textbf{Mesh} & \textbf{Hard-Z} & \textbf{Ours} & \textbf{Diss.} & \textbf{Res.} \\
\addlinespace[0.5pt]

\setboxes{140}{010}{320}{118}{620}{170}{770}{260}
\rotatebox[origin=c]{90}{\textbf{Playroom}} &
\gtbox{images/exp12/playroom/gt.jpg} &
\patchcol{images/exp12/playroom/gt.jpg} &
\patchcol{images/exp12/playroom/mesh.jpg} &
\patchcol{images/exp12/playroom/hardz.jpg} &
\patchcol{images/exp12/playroom/ours.jpg} &
\patchcol{images/exp12/playroom/NDF.png} &
\patchcol{images/exp12/playroom/ResidualContribution.jpg} \\
\addlinespace[4pt]

\setboxes{600}{765}{750}{855}{560}{300}{760}{420}
\rotatebox[origin=c]{90}{\textbf{DrJohnson}} &
\gtbox{images/exp12/DrJohnson/gt.jpg} &
\patchcol{images/exp12/DrJohnson/gt.jpg} &
\patchcol{images/exp12/DrJohnson/mesh.jpg} &
\patchcol{images/exp12/DrJohnson/hardz.jpg} &
\patchcol{images/exp12/DrJohnson/ours.jpg} &
\patchcol{images/exp12/DrJohnson/NDF.png} &
\patchcol{images/exp12/DrJohnson/Residual.jpg} \\
\addlinespace[4pt]

\setboxes{600}{615}{750}{705}{180}{530}{280}{590}
\rotatebox[origin=c]{90}{\textbf{SaintAnne}} &
\gtbox{images/exp12/saintanne/gt.jpg} &
\patchcol{images/exp12/saintanne/gt.jpg} &
\patchcol{images/exp12/saintanne/mesh.jpg} &
\patchcol{images/exp12/saintanne/hardz.jpg} &
\patchcol{images/exp12/saintanne/ours.jpg} &
\patchcol{images/exp12/saintanne/NDF.png} &
\patchcol{images/exp12/saintanne/Residual.jpg} \\
\addlinespace[4pt]



\end{tabular}%
}
\caption{\textbf{Visualization of the subtract-and-refill mechanism.}
Compared with the projection-textured mesh and the Hard-Z hybrid baseline, Gaussolve selectively dissolves inconsistent mesh content (Diss.) and lets residual Gaussians refill the revealed regions (Res.), producing cleaner boundaries and more accurate appearance. The red and blue boxes indicate the corresponding enlarged regions.}
\label{decomposition}
\end{figure*}

==> exp4.tex <==
\begin{figure*}[t]
\centering
\newcommand{\rowlabelwidth}{0.018\linewidth}
\newcommand{\ninefigwidth}{0.106\linewidth}
\newcommand{\cropGroupOne}[1]{\includegraphics[width=\linewidth, trim=0 350 650 178, clip]{#1}}
\newcommand{\cropGroupTwo}[1]{\includegraphics[width=\linewidth, trim=480 355 220 205, clip]{#1}}
\newcommand{\cropGroupThree}[1]{\includegraphics[width=\linewidth, trim=370 310 340 258, clip]{#1}}

\newcommand{\rowlabel}[1]{%
    \makebox[\rowlabelwidth][l]{%
        $\vcenter{\hbox{\rotatebox[origin=c]{90}{\small #1}}}$%
    }%
}

\noindent\makebox[\linewidth][l]{%
    \makebox[\rowlabelwidth]{}%
    \makebox[0.318\linewidth][c]{\small\textbf{Group 1}}\hfill
    \makebox[0.318\linewidth][c]{\small\textbf{Group 2}}\hfill
    \makebox[0.318\linewidth][c]{\small\textbf{Group 3}}%
}
\par\vspace{0mm}

\noindent\makebox[\linewidth][l]{%
    \rowlabel{w/ SH}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupTwo{images/exp4/sh/00023.png_dissolve.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupTwo{images/exp4/sh/00023.png_gs_total.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupTwo{images/exp4/sh/00023.png_blend.jpg} \end{subfigure}%
    \hfill
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupOne{images/exp4/sh/00019.png_dissolve.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupOne{images/exp4/sh/00019.png_gs_total.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupOne{images/exp4/sh/00019.png_blend.jpg} \end{subfigure}%
    \hfill
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupThree{images/exp4/sh/00028.png_dissolve.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupThree{images/exp4/sh/00028.png_gs_total.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupThree{images/exp4/sh/00028.png_blend.jpg} \end{subfigure}%
}

\vspace{0.5mm}


\noindent\makebox[\linewidth][l]{%
    \rowlabel{w/o SH}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupTwo{images/exp4/nosh/00023.png_dissolve.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupTwo{images/exp4/nosh/00023.png_gs_total.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupTwo{images/exp4/nosh/00023.png_blend.jpg} \end{subfigure}%
\hfill
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupOne{images/exp4/nosh/00019.png_dissolve.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupOne{images/exp4/nosh/00019.png_gs_total.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupOne{images/exp4/nosh/00019.png_blend.jpg} \end{subfigure}%
    \hfill
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupThree{images/exp4/nosh/00028.png_dissolve.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupThree{images/exp4/nosh/00028.png_gs_total.jpg} \end{subfigure}%
    \begin{subfigure}[c]{\ninefigwidth} \cropGroupThree{images/exp4/nosh/00028.png_blend.jpg} \end{subfigure}%
}
\vspace{0.1mm}

\caption{\directionalDissolveCaption}
\label{fig:ablation_sh}
\end{figure*}


==> table3.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.08}

\caption{\textbf{Ablation study on ML-Hypersim-001.}
Ablations of representation components, training design, and mesh geometry/appearance.}
\label{tab:ablation}

\begin{tabularx}{\linewidth}{
@{}
>{\hsize=2.5\hsize\raggedright\arraybackslash}X|
c
>{\hsize=0.5\hsize\centering\arraybackslash}X
>{\hsize=0.5\hsize\centering\arraybackslash}X
>{\hsize=0.5\hsize\centering\arraybackslash}X
@{}}
\toprule
Variant & Faces & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule

\multicolumn{5}{@{}l}{\textbf{A. Component Ablation (RC)}} \\
\midrule
Mesh Only
& -- & 27.97 & 0.894 & 0.249 \\

Residual GS Only
& -- & 34.25 & 0.960 & 0.153 \\

Mesh + Residual GS (Hard-Z)
& -- & 33.51 & 0.932 & 0.197 \\

Mesh + NDF
& -- & 29.76 & 0.896 & 0.241 \\

\rowcolor{gray!10}
Full
& -- & \textbf{35.21} & \textbf{0.963} & \textbf{0.106} \\

\midrule
\multicolumn{5}{@{}l}{\textbf{B. Training-Design Ablation (RC)}} \\
\midrule

w/o Scalar SH
& -- & 34.64 & 0.954 & 0.116 \\

w/o Dual Densification
& -- & 34.80 & 0.957 & 0.115 \\

w/o Progressive Initialization
& -- & 35.02 & 0.959 & 0.109 \\

\midrule
\multicolumn{5}{@{}l}{\textbf{C. Geometry and Appearance Ablation (PGSR)}} \\
\midrule

PGSR + Projection
& 10K & 35.52 & 0.963 & 0.112 \\

PGSR + Projection
& 50K & 35.56 & 0.964 & \textbf{0.111} \\

PGSR + Projection
& 100K & \textbf{35.61} & 0.964 & 0.112 \\

PGSR + Projection
& 1M & 35.57 & \textbf{0.965} & 0.112 \\

PGSR + Baked Color
& 100K & 35.42 & 0.961 & 0.140 \\

\bottomrule
\end{tabularx}
\end{table}
